Off-centre ignition of sub-Chandrasekhar white dwarfs does not resolve the tension with the observed $t_0$-$M_{\rm{Ni}56}$ relation of type Ia supernovae

Type Ia supernovae (SNe Ia) are likely the thermonuclear explosions of carbon-oxygen (CO) white-dwarf (WD) stars, but the exact nature of their progenitor systems remains uncertain. Recent studies have suggested that a propagating detonation within a thin helium shell surrounding a sub-Chandrasekhar mass CO core can subsequently trigger a detonation within the core (the double-detonation model, DDM). The resulting explosion resembles a central ignition of a sub-Chandrasekhar mass CO WD (SCD), which is known to be in tension with the observed $t_0$-$M_{\rm{Ni}56}$ relation, where $t_0$ (the $\gamma$-rays' escape time from the ejecta) is positively correlated with $M_{\rm{Ni}56}$ (the synthesized $^{56}$Ni mass). SCD predicts an anticorrelation between $t_0$ and $M_{\rm{Ni}56}$, with $t_0\mathord{\approx}30\,\textrm{day}$ for luminous ($M_{\rm{Ni}56}\gtrsim0.5\,M_{\odot}$) SNe Ia, while the observed $t_0$ is in the range of 35-45 day. In this study, we apply our recently developed numerical scheme to calculate in 2D the impact of off-centre ignition in sub-Chandrasekhar mass CO WD, aiming to better emulate the behaviour expected in the DDM scenario. Our calculations of the $t_0$-$M_{\rm{Ni}56}$ relation, which do not require radiation transfer calculations, achieve convergence to within a few per cent with a numerical resolution of $\mathord{\sim}1\,\rm{km}$. We find that the results only slightly depend on the ignition location, mirroring the SCD model, and consequently, the discrepancy with the observed $t_0$-$M_{\rm{Ni}56}$ relation remains unresolved.

==> restab.tex <==
\clearpage
\onecolumn
\begin{longtable}{lccccccccr}
    \caption{The details of the 2D simulations introduced in this paper. \textbf{Eden: I suggest adding also the loe resolution calculations. You can provide only a few lines for the paper and provide the full table in electronic format}\kushnirq{!Is it fine? I have added also the results of $\zig=0.1$ but they are available only for 1km resolution. I can run other resultions if needed.}}\label{tab:tabres}\\
    \toprule
    $\mwd[\msol]$ & $\zig$ & $\Rig[\rm{km}]$ & $ \Delta x[\rm{km}]$ & $N_{\rm{iso}}$ & $\flim$ & $\mnii[\msol]$ & $t_0[\rm{days}]$ \\
    \midrule
    \endfirsthead
        \caption{continued}\\
    \toprule
    $\mwd[\msol]$ & $\zig$ & $\Rig[\rm{km}]$ & $ \Delta x[\rm{km}]$ & $N_{\rm{iso}}$ & $\flim$ & $\mnii[\msol]$ & $t_0[\rm{days}]$ \\
    \midrule
    \endhead
%\centering
%\caption{The details of the 2D simulations introduced in this paper. \textbf{Eden: I suggest adding also the loe resolution calculations. You can provide only a few lines for the paper and provide the full table in electronic format}\kushnirq{!Is it ok? it made the table too long for a single page so i manually splitted it.}}
%\begin{tabular}{lccccccccr} % four columns, alignment for each
%\hline
%$\mwd[\msol]$ & $\zig$ & $\Rig[\rm{km}]$ & $ \Delta x[\rm{km}]$ & $N_{\rm{iso}}$ & %$\flim$ & $\mnii[\msol]$ & $t_0[\rm{days}]$ \\
$0.80$ & $0.00$ & $1600$ & $16.0$ & $38$ & $0.10$ & $1.20 \times 10^{-1}$ & $32.4$ \\
$0.80$ & $0.00$ & $800$ & $8.0$ & $38$ & $0.10$ & $3.55 \times 10^{-2}$ & $37.0$ \\
$0.80$ & $0.00$ & $400$ & $4.0$ & $38$ & $0.10$ & $2.15 \times 10^{-2}$ & $36.0$ \\
$0.80$ & $0.00$ & $200$ & $2.0$ & $38$ & $0.10$ & $2.70 \times 10^{-2}$ & $33.7$ \\
$0.80$ & $0.00$ & $100$ & $1.0$ & $38$ & $0.10$ & $3.33 \times 10^{-2}$ & $33.5$ \\
$0.80$ & $0.00$ & $100$ & $1.0$ & $69$ & $0.10$ & $3.05 \times 10^{-2}$ & $32.8$ \\
$0.80$ & $0.00$ & $50$ & $0.5$ & $38$ & $0.10$ & $3.73 \times 10^{-2}$ & $33.3$ \\
$0.85$ & $0.00$ & $1600$ & $16.0$ & $38$ & $0.10$ & $1.90 \times 10^{-1}$ & $32.3$ \\
$0.85$ & $0.00$ & $800$ & $8.0$ & $38$ & $0.10$ & $8.33 \times 10^{-2}$ & $35.7$ \\
$0.85$ & $0.00$ & $400$ & $4.0$ & $38$ & $0.10$ & $5.34 \times 10^{-2}$ & $35.4$ \\
$0.85$ & $0.00$ & $200$ & $2.0$ & $38$ & $0.10$ & $6.36 \times 10^{-2}$ & $34.3$ \\
$0.85$ & $0.00$ & $100$ & $1.0$ & $38$ & $0.10$ & $8.88 \times 10^{-2}$ & $33.9$ \\
$0.85$ & $0.00$ & $50$ & $0.5$ & $38$ & $0.10$ & $1.11 \times 10^{-1}$ & $33.8$ \\
$0.90$ & $0.00$ & $1600$ & $16.0$ & $38$ & $0.10$ & $2.93 \times 10^{-1}$ & $32.1$ \\
$0.90$ & $0.00$ & $800$ & $8.0$ & $38$ & $0.10$ & $1.82 \times 10^{-1}$ & $34.4$ \\
$0.90$ & $0.00$ & $400$ & $4.0$ & $38$ & $0.10$ & $1.64 \times 10^{-1}$ & $34.5$ \\
$0.90$ & $0.00$ & $200$ & $2.0$ & $38$ & $0.10$ & $2.06 \times 10^{-1}$ & $33.5$ \\
$0.90$ & $0.00$ & $100$ & $1.0$ & $38$ & $0.10$ & $2.35 \times 10^{-1}$ & $33.0$ \\
$0.90$ & $0.00$ & $50$ & $0.5$ & $38$ & $0.10$ & $2.52 \times 10^{-1}$ & $32.8$ \\
$0.95$ & $0.00$ & $1600$ & $16.0$ & $38$ & $0.10$ & $4.22 \times 10^{-1}$ & $31.8$ \\
$0.95$ & $0.00$ & $800$ & $8.0$ & $38$ & $0.10$ & $3.25 \times 10^{-1}$ & $33.1$ \\
$0.95$ & $0.00$ & $400$ & $4.0$ & $38$ & $0.10$ & $3.32 \times 10^{-1}$ & $32.9$ \\
$0.95$ & $0.00$ & $200$ & $2.0$ & $38$ & $0.10$ & $3.67 \times 10^{-1}$ & $32.3$ \\
$0.95$ & $0.00$ & $100$ & $1.0$ & $38$ & $0.10$ & $3.89 \times 10^{-1}$ & $32.0$ \\
$1.00$ & $0.00$ & $1600$ & $16.0$ & $38$ & $0.10$ & $5.62 \times 10^{-1}$ & $31.7$ \\
$1.00$ & $0.00$ & $800$ & $8.0$ & $38$ & $0.10$ & $4.84 \times 10^{-1}$ & $32.0$ \\
$1.00$ & $0.00$ & $400$ & $4.0$ & $38$ & $0.10$ & $4.96 \times 10^{-1}$ & $31.8$ \\
$1.00$ & $0.00$ & $200$ & $2.0$ & $38$ & $0.10$ & $5.23 \times 10^{-1}$ & $31.4$ \\
$1.00$ & $0.00$ & $100$ & $1.0$ & $38$ & $0.10$ & $5.37 \times 10^{-1}$ & $31.2$ \\
$1.10$ & $0.00$ & $1600$ & $16.0$ & $38$ & $0.10$ & $8.26 \times 10^{-1}$ & $32.6$ \\
$1.10$ & $0.00$ & $800$ & $8.0$ & $38$ & $0.10$ & $7.88 \times 10^{-1}$ & $30.8$ \\
$1.10$ & $0.00$ & $400$ & $4.0$ & $38$ & $0.10$ & $7.80 \times 10^{-1}$ & $30.7$ \\
$1.10$ & $0.00$ & $200$ & $2.0$ & $38$ & $0.10$ & $7.94 \times 10^{-1}$ & $30.4$ \\
$1.10$ & $0.00$ & $100$ & $1.0$ & $38$ & $0.10$ & $8.01 \times 10^{-1}$ & $30.3$ \\
$1.10$ & $0.00$ & $100$ & $1.0$ & $69$ & $0.10$ & $7.93 \times 10^{-1}$ & $30.3$ \\
$0.80$ & $0.00$ & $3200$ & $16.0$ & $38$ & $0.05$ & $3.82 \times 10^{-1}$ & $23.8$ \\
$0.80$ & $0.00$ & $1600$ & $8.0$ & $38$ & $0.05$ & $1.28 \times 10^{-1}$ & $32.2$ \\
$0.80$ & $0.00$ & $800$ & $4.0$ & $38$ & $0.05$ & $3.97 \times 10^{-2}$ & $36.7$ \\
$0.80$ & $0.00$ & $400$ & $2.0$ & $38$ & $0.05$ & $2.14 \times 10^{-2}$ & $36.2$ \\
$0.80$ & $0.00$ & $200$ & $1.0$ & $38$ & $0.05$ & $2.30 \times 10^{-2}$ & $34.6$ \\
$0.80$ & $0.00$ & $100$ & $0.5$ & $38$ & $0.05$ & $2.90 \times 10^{-2}$ & $33.8$ \\
$1.10$ & $0.00$ & $3200$ & $16.0$ & $38$ & $0.05$ & $9.32 \times 10^{-1}$ & $22.7$ \\
$1.10$ & $0.00$ & $1600$ & $8.0$ & $38$ & $0.05$ & $8.45 \times 10^{-1}$ & $32.4$ \\
$1.10$ & $0.00$ & $800$ & $4.0$ & $38$ & $0.05$ & $7.98 \times 10^{-1}$ & $30.7$ \\
$1.10$ & $0.00$ & $400$ & $2.0$ & $38$ & $0.05$ & $7.83 \times 10^{-1}$ & $30.6$ \\
$1.10$ & $0.00$ & $200$ & $1.0$ & $38$ & $0.05$ & $7.94 \times 10^{-1}$ & $30.4$ \\
$0.80$ & $0.10$ & $200$ & $2.0$ & $38$ & $0.10$ & $2.74 \times 10^{-2}$ & $33.9$ \\
$0.80$ & $0.10$ & $100$ & $1.0$ & $38$ & $0.10$ & $3.41 \times 10^{-2}$ & $33.6$ \\
$0.80$ & $0.10$ & $50$ & $0.5$ & $38$ & $0.10$ & $3.43 \times 10^{-2}$ & $33.5$ \\
$0.85$ & $0.10$ & $200$ & $2.0$ & $38$ & $0.10$ & $7.20 \times 10^{-2}$ & $34.4$ \\
$0.85$ & $0.10$ & $100$ & $1.0$ & $38$ & $0.10$ & $9.63 \times 10^{-2}$ & $34.0$ \\
$0.85$ & $0.10$ & $50$ & $0.5$ & $38$ & $0.10$ & $1.13 \times 10^{-1}$ & $33.8$ \\
$0.90$ & $0.10$ & $200$ & $2.0$ & $38$ & $0.10$ & $2.04 \times 10^{-1}$ & $33.6$ \\
$0.90$ & $0.10$ & $100$ & $1.0$ & $38$ & $0.10$ & $2.34 \times 10^{-1}$ & $33.0$ \\
$0.90$ & $0.10$ & $50$ & $0.5$ & $38$ & $0.10$ & $2.52 \times 10^{-1}$ & $32.8$ \\
$0.95$ & $0.10$ & $200$ & $2.0$ & $38$ & $0.10$ & $3.66 \times 10^{-1}$ & $32.3$ \\
$0.95$ & $0.10$ & $100$ & $1.0$ & $38$ & $0.10$ & $3.88 \times 10^{-1}$ & $32.0$ \\
$1.00$ & $0.10$ & $200$ & $2.0$ & $38$ & $0.10$ & $5.20 \times 10^{-1}$ & $31.4$ \\
$1.00$ & $0.10$ & $100$ & $1.0$ & $38$ & $0.10$ & $5.36 \times 10^{-1}$ & $31.2$ \\
$1.10$ & $0.10$ & $200$ & $2.0$ & $38$ & $0.10$ & $7.93 \times 10^{-1}$ & $30.4$ \\
$1.10$ & $0.10$ & $100$ & $1.0$ & $38$ & $0.10$ & $8.01 \times 10^{-1}$ & $30.3$ \\
$0.80$ & $0.25$ & $1600$ & $16.0$ & $38$ & $0.10$ & $9.72 \times 10^{-2}$ & $30.4$ \\
$0.80$ & $0.25$ & $800$ & $8.0$ & $38$ & $0.10$ & $2.66 \times 10^{-2}$ & $33.6$ \\
$0.80$ & $0.25$ & $400$ & $4.0$ & $38$ & $0.10$ & $2.30 \times 10^{-2}$ & $35.4$ \\
$0.80$ & $0.25$ & $200$ & $2.0$ & $38$ & $0.10$ & $3.21 \times 10^{-2}$ & $34.3$ \\
$0.80$ & $0.25$ & $100$ & $1.0$ & $38$ & $0.10$ & $4.04 \times 10^{-2}$ & $33.8$ \\
$0.80$ & $0.25$ & $50$ & $0.5$ & $38$ & $0.10$ & $4.69 \times 10^{-2}$ & $33.9$ \\
$0.85$ & $0.25$ & $1600$ & $16.0$ & $38$ & $0.10$ & $1.69 \times 10^{-1}$ & $31.4$ \\
$0.85$ & $0.25$ & $800$ & $8.0$ & $38$ & $0.10$ & $6.89 \times 10^{-2}$ & $34.9$ \\
$0.85$ & $0.25$ & $400$ & $4.0$ & $38$ & $0.10$ & $6.94 \times 10^{-2}$ & $35.2$ \\
$0.85$ & $0.25$ & $200$ & $2.0$ & $38$ & $0.10$ & $9.62 \times 10^{-2}$ & $34.4$ \\
$0.85$ & $0.25$ & $100$ & $1.0$ & $38$ & $0.10$ & $1.16 \times 10^{-1}$ & $33.9$ \\
$0.85$ & $0.25$ & $50$ & $0.5$ & $38$ & $0.10$ & $1.28 \times 10^{-1}$ & $33.8$ \\
$0.90$ & $0.25$ & $1600$ & $16.0$ & $38$ & $0.10$ & $2.76 \times 10^{-1}$ & $31.5$ \\
$0.90$ & $0.25$ & $800$ & $8.0$ & $38$ & $0.10$ & $1.80 \times 10^{-1}$ & $34.1$ \\
$0.90$ & $0.25$ & $400$ & $4.0$ & $38$ & $0.10$ & $1.85 \times 10^{-1}$ & $34.1$ \\
$0.90$ & $0.25$ & $200$ & $2.0$ & $38$ & $0.10$ & $2.15 \times 10^{-1}$ & $33.4$ \\
$0.90$ & $0.25$ & $100$ & $1.0$ & $38$ & $0.10$ & $2.40 \times 10^{-1}$ & $32.9$ \\
$0.90$ & $0.25$ & $50$ & $0.5$ & $38$ & $0.10$ & $2.53 \times 10^{-1}$ & $32.7$ \\
$0.95$ & $0.25$ & $1600$ & $16.0$ & $38$ & $0.10$ & $4.07 \times 10^{-1}$ & $31.2$ \\
$0.95$ & $0.25$ & $800$ & $8.0$ & $38$ & $0.10$ & $3.25 \times 10^{-1}$ & $32.9$ \\
$0.95$ & $0.25$ & $400$ & $4.0$ & $38$ & $0.10$ & $3.34 \times 10^{-1}$ & $32.8$ \\
$0.95$ & $0.25$ & $200$ & $2.0$ & $38$ & $0.10$ & $3.61 \times 10^{-1}$ & $32.3$ \\
$0.95$ & $0.25$ & $100$ & $1.0$ & $38$ & $0.10$ & $3.83 \times 10^{-1}$ & $31.9$ \\
$1.00$ & $0.25$ & $1600$ & $16.0$ & $38$ & $0.10$ & $5.46 \times 10^{-1}$ & $30.9$ \\
$1.00$ & $0.25$ & $800$ & $8.0$ & $38$ & $0.10$ & $4.78 \times 10^{-1}$ & $31.9$ \\
$1.00$ & $0.25$ & $400$ & $4.0$ & $38$ & $0.10$ & $4.89 \times 10^{-1}$ & $31.8$ \\
$1.00$ & $0.25$ & $200$ & $2.0$ & $38$ & $0.10$ & $5.12 \times 10^{-1}$ & $31.4$ \\
$1.00$ & $0.25$ & $100$ & $1.0$ & $38$ & $0.10$ & $5.29 \times 10^{-1}$ & $31.2$ \\
$1.10$ & $0.25$ & $1600$ & $16.0$ & $38$ & $0.10$ & $8.11 \times 10^{-1}$ & $30.8$ \\
$1.10$ & $0.25$ & $800$ & $8.0$ & $38$ & $0.10$ & $7.68 \times 10^{-1}$ & $30.7$ \\
$1.10$ & $0.25$ & $400$ & $4.0$ & $38$ & $0.10$ & $7.72 \times 10^{-1}$ & $30.6$ \\
$1.10$ & $0.25$ & $200$ & $2.0$ & $38$ & $0.10$ & $7.86 \times 10^{-1}$ & $30.3$ \\
$1.10$ & $0.25$ & $100$ & $1.0$ & $38$ & $0.10$ & $7.97 \times 10^{-1}$ & $30.2$ \\
$0.80$ & $0.50$ & $1600$ & $16.0$ & $38$ & $0.10$ & $3.87 \times 10^{-2}$ & $24.6$ \\
$0.80$ & $0.50$ & $800$ & $8.0$ & $38$ & $0.10$ & $2.11 \times 10^{-2}$ & $34.3$ \\
$0.80$ & $0.50$ & $400$ & $4.0$ & $38$ & $0.10$ & $2.60 \times 10^{-2}$ & $36.5$ \\
$0.80$ & $0.50$ & $200$ & $2.0$ & $38$ & $0.10$ & $3.77 \times 10^{-2}$ & $36.5$ \\
$0.80$ & $0.50$ & $200$ & $1.0$ & $38$ & $0.10$ & $4.86 \times 10^{-2}$ & $36.1$ \\
$0.80$ & $0.50$ & $200$ & $1.0$ & $69$ & $0.10$ & $5.93 \times 10^{-2}$ & $35.8$ \\
$0.80$ & $0.50$ & $200$ & $0.5$ & $38$ & $0.10$ & $5.49 \times 10^{-2}$ & $36.1$ \\
$0.85$ & $0.50$ & $1600$ & $16.0$ & $38$ & $0.10$ & $8.13 \times 10^{-2}$ & $28.9$ \\
$0.85$ & $0.50$ & $800$ & $8.0$ & $38$ & $0.10$ & $6.54 \times 10^{-2}$ & $35.1$ \\
$0.85$ & $0.50$ & $400$ & $4.0$ & $38$ & $0.10$ & $9.32 \times 10^{-2}$ & $35.1$ \\
$0.85$ & $0.50$ & $200$ & $2.0$ & $38$ & $0.10$ & $1.16 \times 10^{-1}$ & $34.9$ \\
$0.85$ & $0.50$ & $100$ & $1.0$ & $38$ & $0.10$ & $1.35 \times 10^{-1}$ & $35.3$ \\
$0.85$ & $0.50$ & $100$ & $0.5$ & $38$ & $0.10$ & $1.44 \times 10^{-1}$ & $33.8$ \\
$0.90$ & $0.50$ & $1600$ & $16.0$ & $38$ & $0.10$ & $2.01 \times 10^{-1}$ & $31.0$ \\
$0.90$ & $0.50$ & $800$ & $8.0$ & $38$ & $0.10$ & $1.73 \times 10^{-1}$ & $33.9$ \\
$0.90$ & $0.50$ & $400$ & $4.0$ & $38$ & $0.10$ & $2.11 \times 10^{-1}$ & $33.8$ \\
$0.90$ & $0.50$ & $200$ & $2.0$ & $38$ & $0.10$ & $2.34 \times 10^{-1}$ & $33.4$ \\
$0.90$ & $0.50$ & $100$ & $1.0$ & $38$ & $0.10$ & $2.55 \times 10^{-1}$ & $33.0$ \\
$0.90$ & $0.50$ & $50$ & $0.5$ & $38$ & $0.10$ & $2.62 \times 10^{-1}$ & $32.6$ \\
$0.95$ & $0.50$ & $1600$ & $16.0$ & $38$ & $0.10$ & $3.51 \times 10^{-1}$ & $30.8$ \\
$0.95$ & $0.50$ & $800$ & $8.0$ & $38$ & $0.10$ & $3.11 \times 10^{-1}$ & $32.7$ \\
$0.95$ & $0.50$ & $400$ & $4.0$ & $38$ & $0.10$ & $3.46 \times 10^{-1}$ & $32.6$ \\
$0.95$ & $0.50$ & $200$ & $2.0$ & $38$ & $0.10$ & $3.73 \times 10^{-1}$ & $32.1$ \\
$0.95$ & $0.50$ & $100$ & $1.0$ & $38$ & $0.10$ & $3.90 \times 10^{-1}$ & $31.9$ \\
$1.00$ & $0.50$ & $1600$ & $16.0$ & $38$ & $0.10$ & $5.03 \times 10^{-1}$ & $30.2$ \\
$1.00$ & $0.50$ & $800$ & $8.0$ & $38$ & $0.10$ & $4.65 \times 10^{-1}$ & $31.6$ \\
$1.00$ & $0.50$ & $400$ & $4.0$ & $38$ & $0.10$ & $4.86 \times 10^{-1}$ & $31.6$ \\
$1.00$ & $0.50$ & $200$ & $2.0$ & $38$ & $0.10$ & $5.10 \times 10^{-1}$ & $31.3$ \\
$1.00$ & $0.50$ & $100$ & $1.0$ & $38$ & $0.10$ & $5.26 \times 10^{-1}$ & $31.1$ \\
$1.10$ & $0.50$ & $1600$ & $16.0$ & $38$ & $0.10$ & $7.81 \times 10^{-1}$ & $29.4$ \\
$1.10$ & $0.50$ & $800$ & $8.0$ & $38$ & $0.10$ & $7.50 \times 10^{-1}$ & $30.4$ \\
$1.10$ & $0.50$ & $400$ & $4.0$ & $38$ & $0.10$ & $7.58 \times 10^{-1}$ & $30.3$ \\
$1.10$ & $0.50$ & $200$ & $2.0$ & $38$ & $0.10$ & $7.71 \times 10^{-1}$ & $30.2$ \\
$1.10$ & $0.50$ & $100$ & $1.0$ & $38$ & $0.10$ & $7.83 \times 10^{-1}$ & $30.0$ \\
$1.10$ & $0.50$ & $100$ & $1.0$ & $69$ & $0.10$ & $7.75 \times 10^{-1}$ & $30.0$ \\
$0.80$ & $0.50$ & $3200$ & $16.0$ & $38$ & $0.05$ & $1.72 \times 10^{-1}$ & $20.7$ \\
$0.80$ & $0.50$ & $1600$ & $8.0$ & $38$ & $0.05$ & $4.06 \times 10^{-2}$ & $24.9$ \\
$0.80$ & $0.50$ & $800$ & $4.0$ & $38$ & $0.05$ & $2.21 \times 10^{-2}$ & $34.5$ \\
$0.80$ & $0.50$ & $400$ & $2.0$ & $38$ & $0.05$ & $2.58 \times 10^{-2}$ & $36.4$ \\
$0.80$ & $0.50$ & $200$ & $1.0$ & $38$ & $0.05$ & $3.61 \times 10^{-2}$ & $36.7$ \\
$0.80$ & $0.50$ & $200$ & $0.5$ & $38$ & $0.05$ & $4.34 \times 10^{-2}$ & $36.6$ \\
$1.10$ & $0.50$ & $3200$ & $16.0$ & $38$ & $0.05$ & $8.92 \times 10^{-1}$ & $26.1$ \\
$1.10$ & $0.50$ & $1600$ & $8.0$ & $38$ & $0.05$ & $7.97 \times 10^{-1}$ & $29.2$ \\
$1.10$ & $0.50$ & $800$ & $4.0$ & $38$ & $0.05$ & $7.59 \times 10^{-1}$ & $30.3$ \\
$1.10$ & $0.50$ & $400$ & $2.0$ & $38$ & $0.05$ & $7.63 \times 10^{-1}$ & $30.3$ \\
$1.10$ & $0.50$ & $200$ & $1.0$ & $38$ & $0.05$ & $7.73 \times 10^{-1}$ & $30.2$ \\
$0.80$ & $0.75$ & $1600$ & $8.0$ & $38$ & $0.10$ & $2.71 \times 10^{-2}$ & $32.4$ \\
$0.80$ & $0.75$ & $800$ & $4.0$ & $38$ & $0.10$ & $3.16 \times 10^{-2}$ & $37.8$ \\
$0.80$ & $0.75$ & $800$ & $2.0$ & $38$ & $0.10$ & $4.63 \times 10^{-2}$ & $36.9$ \\
$0.80$ & $0.75$ & $800$ & $1.0$ & $38$ & $0.10$ & $5.71 \times 10^{-2}$ & $35.2$ \\
$0.80$ & $0.75$ & $400$ & $0.5$ & $38$ & $0.10$ & $5.89 \times 10^{-2}$ & $35.0$ \\
$0.85$ & $0.75$ & $1600$ & $8.0$ & $38$ & $0.10$ & $8.52 \times 10^{-2}$ & $33.1$ \\
$0.85$ & $0.75$ & $800$ & $4.0$ & $38$ & $0.10$ & $1.04 \times 10^{-1}$ & $35.6$ \\
$0.85$ & $0.75$ & $800$ & $2.0$ & $38$ & $0.10$ & $1.31 \times 10^{-1}$ & $35.2$ \\
$0.85$ & $0.75$ & $800$ & $1.0$ & $38$ & $0.10$ & $1.46 \times 10^{-1}$ & $34.0$ \\
$0.85$ & $0.75$ & $400$ & $0.5$ & $38$ & $0.10$ & $1.31 \times 10^{-1}$ & $33.7$ \\
$0.90$ & $0.75$ & $1600$ & $8.0$ & $38$ & $0.10$ & $2.01 \times 10^{-1}$ & $32.6$ \\
$0.90$ & $0.75$ & $800$ & $4.0$ & $38$ & $0.10$ & $2.19 \times 10^{-1}$ & $33.6$ \\
$0.90$ & $0.75$ & $400$ & $2.0$ & $38$ & $0.10$ & $2.41 \times 10^{-1}$ & $33.9$ \\
$0.90$ & $0.75$ & $800$ & $1.0$ & $38$ & $0.10$ & $2.68 \times 10^{-1}$ & $32.1$ \\
$0.90$ & $0.75$ & $400$ & $0.5$ & $38$ & $0.10$ & $2.75 \times 10^{-1}$ & $32.2$ \\
$0.95$ & $0.75$ & $1600$ & $8.0$ & $38$ & $0.10$ & $3.51 \times 10^{-1}$ & $31.4$ \\
$0.95$ & $0.75$ & $800$ & $4.0$ & $38$ & $0.10$ & $3.56 \times 10^{-1}$ & $32.1$ \\
$0.95$ & $0.75$ & $400$ & $2.0$ & $38$ & $0.10$ & $3.76 \times 10^{-1}$ & $32.5$ \\
$0.95$ & $0.75$ & $400$ & $1.0$ & $38$ & $0.10$ & $3.92 \times 10^{-1}$ & $31.9$ \\
$1.00$ & $0.75$ & $1600$ & $8.0$ & $38$ & $0.10$ & $5.05 \times 10^{-1}$ & $30.4$ \\
$1.00$ & $0.75$ & $800$ & $4.0$ & $38$ & $0.10$ & $4.91 \times 10^{-1}$ & $31.3$ \\
$1.00$ & $0.75$ & $400$ & $2.0$ & $38$ & $0.10$ & $5.10 \times 10^{-1}$ & $31.4$ \\
$1.00$ & $0.75$ & $200$ & $1.0$ & $38$ & $0.10$ & $5.21 \times 10^{-1}$ & $31.0$ \\
$1.10$ & $0.75$ & $1600$ & $8.0$ & $38$ & $0.10$ & $7.87 \times 10^{-1}$ & $29.2$ \\
$1.10$ & $0.75$ & $800$ & $4.0$ & $38$ & $0.10$ & $7.57 \times 10^{-1}$ & $30.1$ \\
$1.10$ & $0.75$ & $400$ & $2.0$ & $38$ & $0.10$ & $7.67 \times 10^{-1}$ & $30.0$ \\
$1.10$ & $0.75$ & $200$ & $1.0$ & $38$ & $0.10$ & $7.78 \times 10^{-1}$ & $30.0$ \\
\hline
%\end{tabular}
\end{longtable}
